Two Different Weak Modulations in ab-type RR Lyrae Variable V838 Cyg, and Potential Influence of Metal Abundance on Blazhko Modulation

Noting the weakest modulation and relatively high metal abundance of the ab-type RR Lyrae star V838 Cyg, we collected the photometric data of this star from several sky surveys to carry out an in-depth analysis. The O-C diagram shows that the pulsation period of V838 Cyg increases linearly over a long timescale. In a reanalysis of the high-precision Kepler data, we confirmed the modulation with a period of 59.45\pm0.07 days found by Benko et al., (2014), and also found an additional weak modulation with a longer period (840\pm21 days). After a series of analyses, we incline to the view that the mechanisms causing the two modulations are different: the former is more similar to the typical Blazhko effect, while the mechanism leading to the latter may be an extrinsic factor. We also collected and compared the modulation and physical parameters of other Blazhko RR Lyrae stars from several works in the literature, and find that there is a potential negative correlation between the modulation amplitude (or upper limit of amplitude) and the metal abundance. We infer that the relatively high metal abundance will promote convection in the outer stellar atmosphere, and then inhibit those factors (turbulence, shock wave, etc.) that may cause Blazhko modulation. Future observations and research work can be carried out with reference to this viewpoint. We also introduce the moire effects that appear in the Kepler long-cadence light curves and their possible interference in the previous analyses.

==> data_full_table_and_supplementary_data/Table01_full <==
\begin{table}
\begin{center}
\caption{Times of light maximum and corresponding errors for V838 Cyg provided by present paper. The epoch number and the $O-C$ values are calculated by Equation (3).}\label{Table1}
\begin{tabular}{c c c r c}
\hline\hline
   Max.	       &	Error	  &	Epoch Number	&  $O-C$ & Ref.	\\
HJD-2400000    &	(days)	&		            &	       &      \\
\hline
54231.66773 	&	0.00161 	&	-1526	&	0.00176 	&	SWASP	\\
54232.62931 	&	0.00126 	&	-1524	&	0.00278 	&	SWASP	\\
54256.64342 	&	0.00083 	&	-1474	&	0.00290 	&	SWASP	\\
54257.60145 	&	0.00194 	&	-1472	&	0.00036 	&	SWASP	\\
54280.65827 	&	0.00228 	&	-1424	&	0.00375 	&	SWASP	\\
54282.57607 	&	0.00259 	&	-1420	&	0.00042 	&	SWASP	\\
54283.53631 	&	0.00219 	&	-1418	&	0.00011 	&	SWASP	\\
54284.50162 	&	0.00213 	&	-1416	&	0.00485 	&	SWASP	\\
54609.64631 	&	0.00158 	&	-739	&	0.00005 	&	SWASP	\\
54635.58402 	&	0.00167 	&	-685	&	0.00266 	&	SWASP	\\
54645.66880 	&	0.00221 	&	-664	&	0.00155 	&	SWASP	\\
54646.62835 	&	0.00127 	&	-662	&	0.00054 	&	SWASP	\\
54647.58883 	&	0.00079 	&	-660	&	0.00046 	&	SWASP	\\
54648.55043 	&	0.00235 	&	-658	&	0.00150 	&	SWASP	\\
54659.59704 	&	0.00102 	&	-635	&	0.00167 	&	SWASP	\\
54660.55400 	&	0.00023 	&	-633	&	-0.00193 	&	SWASP	\\
54661.51873 	&	0.00154 	&	-631	&	0.00225 	&	SWASP	\\
54662.47904 	&	0.00191 	&	-629	&	0.00200 	&	SWASP	\\
54663.43947 	&	0.00116 	&	-627	&	0.00187 	&	SWASP	\\
54671.60423 	&	0.00137 	&	-610	&	0.00187 	&	SWASP	\\
54674.48298 	&	0.00079 	&	-604	&	-0.00106 	&	SWASP	\\
54675.44209 	&	0.00040 	&	-602	&	-0.00251 	&	SWASP	\\
54676.40547 	&	0.00102 	&	-600	&	0.00031 	&	SWASP	\\
54685.53175 	&	0.00173 	&	-581	&	0.00127 	&	SWASP	\\
54688.41227 	&	0.00160 	&	-575	&	0.00012 	&	SWASP	\\
54965.05584 	&	0.00011 	&	1	&	0.00246 	&	Kepler	\\
54966.49636 	&	0.00008 	&	4	&	0.00214 	&	Kepler	\\
54967.93746 	&	0.00006 	&	7	&	0.00240 	&	Kepler	\\
54969.85864 	&	0.00008 	&	11	&	0.00246 	&	Kepler	\\
54971.29934 	&	0.00007 	&	14	&	0.00232 	&	Kepler	\\
54972.74025 	&	0.00010 	&	17	&	0.00239 	&	Kepler	\\
54974.18103 	&	0.00007 	&	20	&	0.00233 	&	Kepler	\\
54975.62202 	&	0.00009 	&	23	&	0.00248 	&	Kepler	\\
54977.06264 	&	0.00008 	&	26	&	0.00227 	&	Kepler	\\
54978.50360 	&	0.00006 	&	29	&	0.00238 	&	Kepler	\\
54979.94440 	&	0.00008 	&	32	&	0.00235 	&	Kepler	\\
54981.38524 	&	0.00007 	&	35	&	0.00234 	&	Kepler	\\
54982.82604 	&	0.00007 	&	38	&	0.00230 	&	Kepler	\\
54984.26686 	&	0.00005 	&	41	&	0.00228 	&	Kepler	\\
54986.18810 	&	0.00008 	&	45	&	0.00241 	&	Kepler	\\
54987.62878 	&	0.00008 	&	48	&	0.00225 	&	Kepler	\\
54989.54977 	&	0.00028 	&	52	&	0.00212 	&	Kepler	\\
54990.99077 	&	0.00005 	&	55	&	0.00228 	&	Kepler	\\
54992.43122 	&	0.00020 	&	58	&	0.00189 	&	Kepler	\\
54993.87251 	&	0.00005 	&	61	&	0.00234 	&	Kepler	\\
54996.27380 	&	0.00005 	&	66	&	0.00223 	&	Kepler	\\
55001.07702 	&	0.00005 	&	76	&	0.00265 	&	Kepler	\\
55004.91850 	&	0.00009 	&	84	&	0.00189 	&	Kepler	\\
55006.36000 	&	0.00054 	&	87	&	0.00255 	&	Kepler	\\
55007.80036 	&	0.00006 	&	90	&	0.00207 	&	Kepler	\\
55009.72159 	&	0.00008 	&	94	&	0.00218 	&	Kepler	\\
55011.16265 	&	0.00007 	&	97	&	0.00240 	&	Kepler	\\
55012.60346 	&	0.00007 	&	100	&	0.00237 	&	Kepler	\\
55015.48507 	&	0.00023 	&	106	&	0.00230 	&	Kepler	\\
55018.36665 	&	0.00018 	&	112	&	0.00220 	&	Kepler	\\
55019.80764 	&	0.00009 	&	115	&	0.00235 	&	Kepler	\\
55021.24842 	&	0.00028 	&	118	&	0.00229 	&	Kepler	\\
55022.68949 	&	0.00024 	&	121	&	0.00253 	&	Kepler	\\
55026.05140 	&	0.00009 	&	128	&	0.00248 	&	Kepler	\\
55027.49205 	&	0.00012 	&	131	&	0.00228 	&	Kepler	\\
55028.93305 	&	0.00011 	&	134	&	0.00245 	&	Kepler	\\
55030.85370 	&	0.00009 	&	138	&	0.00197 	&	Kepler	\\
55032.29480 	&	0.00010 	&	141	&	0.00223 	&	Kepler	\\
55033.73575 	&	0.00004 	&	144	&	0.00234 	&	Kepler	\\
55035.65688 	&	0.00009 	&	148	&	0.00235 	&	Kepler	\\
55037.09805 	&	0.00013 	&	151	&	0.00269 	&	Kepler	\\
55039.01854 	&	0.00009 	&	155	&	0.00206 	&	Kepler	\\
55040.45967 	&	0.00007 	&	158	&	0.00235 	&	Kepler	\\
55041.90032 	&	0.00008 	&	161	&	0.00216 	&	Kepler	\\
55043.34125 	&	0.00007 	&	164	&	0.00225 	&	Kepler	\\
55045.26246 	&	0.00005 	&	168	&	0.00234 	&	Kepler	\\
55046.70324 	&	0.00008 	&	171	&	0.00227 	&	Kepler	\\
55048.14412 	&	0.00007 	&	174	&	0.00232 	&	Kepler	\\
55049.58468 	&	0.00008 	&	177	&	0.00204 	&	Kepler	\\
55051.02554 	&	0.00007 	&	180	&	0.00206 	&	Kepler	\\
55052.94656 	&	0.00005 	&	184	&	0.00196 	&	Kepler	\\
55054.38752 	&	0.00007 	&	187	&	0.00208 	&	Kepler	\\
55055.82847 	&	0.00007 	&	190	&	0.00219 	&	Kepler	\\
55057.74995 	&	0.00005 	&	194	&	0.00254 	&	Kepler	\\
55059.19036 	&	0.00011 	&	197	&	0.00212 	&	Kepler	\\
55060.63138 	&	0.00007 	&	200	&	0.00230 	&	Kepler	\\
55062.07212 	&	0.00006 	&	203	&	0.00220 	&	Kepler	\\
55064.47335 	&	0.00007 	&	208	&	0.00203 	&	Kepler	\\
55066.39469 	&	0.00007 	&	212	&	0.00225 	&	Kepler	\\
55067.83535 	&	0.00008 	&	215	&	0.00208 	&	Kepler	\\
55069.27657 	&	0.00006 	&	218	&	0.00246 	&	Kepler	\\
55070.71709 	&	0.00010 	&	221	&	0.00213 	&	Kepler	\\
55072.15783 	&	0.00009 	&	224	&	0.00203 	&	Kepler	\\
55074.07892 	&	0.00007 	&	228	&	0.00200 	&	Kepler	\\
55077.44106 	&	0.00010 	&	235	&	0.00219 	&	Kepler	\\
55078.88199 	&	0.00008 	&	238	&	0.00228 	&	Kepler	\\
55080.32238 	&	0.00007 	&	241	&	0.00182 	&	Kepler	\\
55081.76369 	&	0.00006 	&	244	&	0.00229 	&	Kepler	\\
55083.68484 	&	0.00012 	&	248	&	0.00233 	&	Kepler	\\
55085.12570 	&	0.00008 	&	251	&	0.00235 	&	Kepler	\\
55087.04670 	&	0.00008 	&	255	&	0.00223 	&	Kepler	\\
55089.44825 	&	0.00007 	&	260	&	0.00238 	&	Kepler	\\
55092.33037 	&	0.00012 	&	266	&	0.00282 	&	Kepler	\\
55094.25075 	&	0.00008 	&	270	&	0.00208 	&	Kepler	\\
55096.17196 	&	0.00006 	&	274	&	0.00216 	&	Kepler	\\
55097.61285 	&	0.00010 	&	277	&	0.00222 	&	Kepler	\\
55099.05321 	&	0.00006 	&	280	&	0.00174 	&	Kepler	\\
55101.93515 	&	0.00006 	&	286	&	0.00200 	&	Kepler	\\
55103.37580 	&	0.00005 	&	289	&	0.00181 	&	Kepler	\\
55105.29751 	&	0.00006 	&	293	&	0.00240 	&	Kepler	\\
55106.73794 	&	0.00013 	&	296	&	0.00199 	&	Kepler	\\
55108.17923 	&	0.00013 	&	299	&	0.00244 	&	Kepler	\\
55109.61972 	&	0.00010 	&	302	&	0.00209 	&	Kepler	\\
55111.06068 	&	0.00011 	&	305	&	0.00221 	&	Kepler	\\
55112.50134 	&	0.00028 	&	308	&	0.00203 	&	Kepler	\\
55114.42268 	&	0.00005 	&	312	&	0.00225 	&	Kepler	\\
55116.34362 	&	0.00012 	&	316	&	0.00207 	&	Kepler	\\
55117.78449 	&	0.00006 	&	319	&	0.00210 	&	Kepler	\\
55119.22549 	&	0.00010 	&	322	&	0.00226 	&	Kepler	\\
55121.14665 	&	0.00006 	&	326	&	0.00230 	&	Kepler	\\
55122.58765 	&	0.00009 	&	329	&	0.00246 	&	Kepler	\\
55124.50837 	&	0.00007 	&	333	&	0.00206 	&	Kepler	\\
55126.42945 	&	0.00011 	&	337	&	0.00203 	&	Kepler	\\
55127.87048 	&	0.00011 	&	340	&	0.00221 	&	Kepler	\\
55129.31130 	&	0.00011 	&	343	&	0.00220 	&	Kepler	\\
55130.75218 	&	0.00010 	&	346	&	0.00224 	&	Kepler	\\
55132.67334 	&	0.00008 	&	350	&	0.00227 	&	Kepler	\\
55134.11403 	&	0.00010 	&	353	&	0.00212 	&	Kepler	\\
55135.55495 	&	0.00010 	&	356	&	0.00220 	&	Kepler	\\
55136.99585 	&	0.00007 	&	359	&	0.00227 	&	Kepler	\\
55138.43673 	&	0.00007 	&	362	&	0.00231 	&	Kepler	\\
55139.87740 	&	0.00006 	&	365	&	0.00214 	&	Kepler	\\
55141.31827 	&	0.00008 	&	368	&	0.00216 	&	Kepler	\\
55142.75910 	&	0.00006 	&	371	&	0.00216 	&	Kepler	\\
55144.20001 	&	0.00005 	&	374	&	0.00222 	&	Kepler	\\
55146.12148 	&	0.00007 	&	378	&	0.00257 	&	Kepler	\\
55147.56212 	&	0.00009 	&	381	&	0.00238 	&	Kepler	\\
55149.00297 	&	0.00006 	&	384	&	0.00238 	&	Kepler	\\
55150.44364 	&	0.00006 	&	387	&	0.00222 	&	Kepler	\\
55151.88453 	&	0.00006 	&	390	&	0.00227 	&	Kepler	\\
55153.32521 	&	0.00028 	&	393	&	0.00211 	&	Kepler	\\
55155.72659 	&	0.00006 	&	398	&	0.00209 	&	Kepler	\\
55158.12818 	&	0.00006 	&	403	&	0.00228 	&	Kepler	\\
55160.04926 	&	0.00008 	&	407	&	0.00224 	&	Kepler	\\
55161.49012 	&	0.00007 	&	410	&	0.00226 	&	Kepler	\\
55162.93072 	&	0.00010 	&	413	&	0.00202 	&	Kepler	\\
55164.37178 	&	0.00007 	&	416	&	0.00224 	&	Kepler	\\
55165.81242 	&	0.00017 	&	419	&	0.00204 	&	Kepler	\\
55167.25344 	&	0.00012 	&	422	&	0.00222 	&	Kepler	\\
55168.69414 	&	0.00013 	&	425	&	0.00208 	&	Kepler	\\
55170.61585 	&	0.00013 	&	429	&	0.00267 	&	Kepler	\\
55172.05615 	&	0.00006 	&	432	&	0.00214 	&	Kepler	\\
55173.49706 	&	0.00010 	&	435	&	0.00221 	&	Kepler	\\
55174.93798 	&	0.00007 	&	438	&	0.00228 	&	Kepler	\\
55176.85905 	&	0.00008 	&	442	&	0.00224 	&	Kepler	\\
55178.29954 	&	0.00009 	&	445	&	0.00188 	&	Kepler	\\
55179.74068 	&	0.00008 	&	448	&	0.00218 	&	Kepler	\\
55181.18165 	&	0.00007 	&	451	&	0.00232 	&	Kepler	\\
55184.06330 	&	0.00012 	&	457	&	0.00229 	&	Kepler	\\
55187.42516 	&	0.00008 	&	464	&	0.00219 	&	Kepler	\\
55188.86608 	&	0.00007 	&	467	&	0.00227 	&	Kepler	\\
55190.30682 	&	0.00009 	&	470	&	0.00217 	&	Kepler	\\
55191.74786 	&	0.00007 	&	473	&	0.00237 	&	Kepler	\\
55193.18850 	&	0.00007 	&	476	&	0.00217 	&	Kepler	\\
55194.62962 	&	0.00006 	&	479	&	0.00244 	&	Kepler	\\
55196.07033 	&	0.00007 	&	482	&	0.00232 	&	Kepler	\\
55197.99166 	&	0.00005 	&	486	&	0.00253 	&	Kepler	\\
55199.43232 	&	0.00005 	&	489	&	0.00235 	&	Kepler	\\
55200.87302 	&	0.00006 	&	492	&	0.00221 	&	Kepler	\\
55202.31381 	&	0.00013 	&	495	&	0.00216 	&	Kepler	\\
55204.23502 	&	0.00007 	&	499	&	0.00225 	&	Kepler	\\
55205.67581 	&	0.00010 	&	502	&	0.00220 	&	Kepler	\\
55207.11718 	&	0.00009 	&	505	&	0.00273 	&	Kepler	\\
55208.55762 	&	0.00009 	&	508	&	0.00233 	&	Kepler	\\
55210.47865 	&	0.00008 	&	512	&	0.00224 	&	Kepler	\\
55211.91921 	&	0.00013 	&	515	&	0.00196 	&	Kepler	\\
55213.84100 	&	0.00011 	&	519	&	0.00263 	&	Kepler	\\
55215.28126 	&	0.00009 	&	522	&	0.00205 	&	Kepler	\\
55217.20261 	&	0.00007 	&	526	&	0.00229 	&	Kepler	\\
55219.12317 	&	0.00113 	&	530	&	0.00172 	&	Kepler	\\
55221.04460 	&	0.00008 	&	534	&	0.00204 	&	Kepler	\\
55222.48565 	&	0.00008 	&	537	&	0.00224 	&	Kepler	\\
55223.92659 	&	0.00011 	&	540	&	0.00235 	&	Kepler	\\
55225.36745 	&	0.00008 	&	543	&	0.00236 	&	Kepler	\\
55226.80834 	&	0.00012 	&	546	&	0.00241 	&	Kepler	\\
55228.24871 	&	0.00011 	&	549	&	0.00194 	&	Kepler	\\
55232.09136 	&	0.00008 	&	557	&	0.00235 	&	Kepler	\\
55235.45304 	&	0.00009 	&	564	&	0.00208 	&	Kepler	\\
55236.89425 	&	0.00012 	&	567	&	0.00244 	&	Kepler	\\
55238.33497 	&	0.00008 	&	570	&	0.00233 	&	Kepler	\\
55239.77573 	&	0.00007 	&	573	&	0.00224 	&	Kepler	\\
55241.21659 	&	0.00007 	&	576	&	0.00227 	&	Kepler	\\
55243.13782 	&	0.00006 	&	580	&	0.00238 	&	Kepler	\\
55244.57855 	&	0.00008 	&	583	&	0.00227 	&	Kepler	\\
55246.01966 	&	0.00007 	&	586	&	0.00253 	&	Kepler	\\
55247.46019 	&	0.00010 	&	589	&	0.00223 	&	Kepler	\\
55248.90104 	&	0.00009 	&	592	&	0.00224 	&	Kepler	\\
55250.82229 	&	0.00005 	&	596	&	0.00237 	&	Kepler	\\
55252.26302 	&	0.00008 	&	599	&	0.00226 	&	Kepler	\\
55253.70422 	&	0.00008 	&	602	&	0.00262 	&	Kepler	\\
55255.14469 	&	0.00005 	&	605	&	0.00225 	&	Kepler	\\
55256.58578 	&	0.00007 	&	608	&	0.00251 	&	Kepler	\\
55258.02616 	&	0.00009 	&	611	&	0.00204 	&	Kepler	\\
55259.46729 	&	0.00008 	&	614	&	0.00233 	&	Kepler	\\
55260.90814 	&	0.00008 	&	617	&	0.00234 	&	Kepler	\\
55262.34909 	&	0.00005 	&	620	&	0.00245 	&	Kepler	\\
55264.27038 	&	0.00004 	&	624	&	0.00262 	&	Kepler	\\
55265.71096 	&	0.00008 	&	627	&	0.00236 	&	Kepler	\\
55267.15205 	&	0.00008 	&	630	&	0.00261 	&	Kepler	\\
55268.59248 	&	0.00007 	&	633	&	0.00220 	&	Kepler	\\
55270.51381 	&	0.00009 	&	637	&	0.00242 	&	Kepler	\\
55271.95472 	&	0.00007 	&	640	&	0.00248 	&	Kepler	\\
55273.39541 	&	0.00009 	&	643	&	0.00233 	&	Kepler	\\
55275.79694 	&	0.00006 	&	648	&	0.00247 	&	Kepler	\\
55278.67841 	&	0.00009 	&	654	&	0.00225 	&	Kepler	\\
55280.11933 	&	0.00008 	&	657	&	0.00233 	&	Kepler	\\
55281.56020 	&	0.00010 	&	660	&	0.00237 	&	Kepler	\\
55283.00091 	&	0.00011 	&	663	&	0.00224 	&	Kepler	\\
55284.44177 	&	0.00007 	&	666	&	0.00225 	&	Kepler	\\
55285.88268 	&	0.00009 	&	669	&	0.00233 	&	Kepler	\\
55287.80362 	&	0.00015 	&	673	&	0.00215 	&	Kepler	\\
55289.24444 	&	0.00007 	&	676	&	0.00213 	&	Kepler	\\
55290.68531 	&	0.00008 	&	679	&	0.00215 	&	Kepler	\\
55292.12613 	&	0.00008 	&	682	&	0.00214 	&	Kepler	\\
55293.56711 	&	0.00009 	&	685	&	0.00228 	&	Kepler	\\
55295.48808 	&	0.00008 	&	689	&	0.00213 	&	Kepler	\\
55296.92907 	&	0.00007 	&	692	&	0.00228 	&	Kepler	\\
55298.36993 	&	0.00007 	&	695	&	0.00230 	&	Kepler	\\
55299.81064 	&	0.00006 	&	698	&	0.00217 	&	Kepler	\\
55301.25141 	&	0.00006 	&	701	&	0.00210 	&	Kepler	\\
55303.17282 	&	0.00005 	&	705	&	0.00239 	&	Kepler	\\
55304.61289 	&	0.00024 	&	708	&	0.00162 	&	Kepler	\\
55306.05409 	&	0.00012 	&	711	&	0.00198 	&	Kepler	\\
55308.45560 	&	0.00005 	&	716	&	0.00209 	&	Kepler	\\
55310.37719 	&	0.00005 	&	720	&	0.00256 	&	Kepler	\\
55311.81779 	&	0.00005 	&	723	&	0.00232 	&	Kepler	\\
55313.25849 	&	0.00005 	&	726	&	0.00218 	&	Kepler	\\
55314.69955 	&	0.00005 	&	729	&	0.00240 	&	Kepler	\\
55316.14034 	&	0.00008 	&	732	&	0.00235 	&	Kepler	\\
55317.58115 	&	0.00006 	&	735	&	0.00233 	&	Kepler	\\
55319.02209 	&	0.00006 	&	738	&	0.00242 	&	Kepler	\\
55320.46266 	&	0.00005 	&	741	&	0.00215 	&	Kepler	\\
55322.38389 	&	0.00010 	&	745	&	0.00226 	&	Kepler	\\
55323.82478 	&	0.00007 	&	748	&	0.00231 	&	Kepler	\\
55325.26583 	&	0.00006 	&	751	&	0.00253 	&	Kepler	\\
55326.70640 	&	0.00006 	&	754	&	0.00226 	&	Kepler	\\
55328.14746 	&	0.00005 	&	757	&	0.00247 	&	Kepler	\\
55329.58804 	&	0.00008 	&	760	&	0.00221 	&	Kepler	\\
55331.02907 	&	0.00007 	&	763	&	0.00240 	&	Kepler	\\
55332.46974 	&	0.00009 	&	766	&	0.00224 	&	Kepler	\\
55333.91076 	&	0.00007 	&	769	&	0.00241 	&	Kepler	\\
55335.35139 	&	0.00009 	&	772	&	0.00221 	&	Kepler	\\
55337.27252 	&	0.00010 	&	776	&	0.00222 	&	Kepler	\\
55338.71317 	&	0.00009 	&	779	&	0.00203 	&	Kepler	\\
55340.15436 	&	0.00008 	&	782	&	0.00238 	&	Kepler	\\
55342.07524 	&	0.00007 	&	786	&	0.00214 	&	Kepler	\\
55343.51614 	&	0.00009 	&	789	&	0.00220 	&	Kepler	\\
55344.95683 	&	0.00010 	&	792	&	0.00205 	&	Kepler	\\
55346.39757 	&	0.00008 	&	795	&	0.00195 	&	Kepler	\\
55347.83840 	&	0.00008 	&	798	&	0.00194 	&	Kepler	\\
55349.27943 	&	0.00009 	&	801	&	0.00213 	&	Kepler	\\
55350.71981 	&	0.00011 	&	804	&	0.00167 	&	Kepler	\\
55352.64143 	&	0.00013 	&	808	&	0.00217 	&	Kepler	\\
55354.08220 	&	0.00009 	&	811	&	0.00210 	&	Kepler	\\
55355.52292 	&	0.00015 	&	814	&	0.00198 	&	Kepler	\\
55356.96394 	&	0.00009 	&	817	&	0.00216 	&	Kepler	\\
55358.40470 	&	0.00010 	&	820	&	0.00208 	&	Kepler	\\
55359.84552 	&	0.00007 	&	823	&	0.00206 	&	Kepler	\\
55361.28651 	&	0.00004 	&	826	&	0.00221 	&	Kepler	\\
55362.72733 	&	0.00009 	&	829	&	0.00219 	&	Kepler	\\
55364.16758 	&	0.00010 	&	832	&	0.00160 	&	Kepler	\\
55366.08936 	&	0.00007 	&	836	&	0.00226 	&	Kepler	\\
55367.53022 	&	0.00016 	&	839	&	0.00228 	&	Kepler	\\
55368.97116 	&	0.00006 	&	842	&	0.00239 	&	Kepler	\\
55371.37238 	&	0.00014 	&	847	&	0.00221 	&	Kepler	\\
55373.77386 	&	0.00006 	&	852	&	0.00229 	&	Kepler	\\
55375.21463 	&	0.00009 	&	855	&	0.00222 	&	Kepler	\\
55376.65563 	&	0.00006 	&	858	&	0.00238 	&	Kepler	\\
55378.09637 	&	0.00006 	&	861	&	0.00228 	&	Kepler	\\
55380.01743 	&	0.00004 	&	865	&	0.00221 	&	Kepler	\\
55381.45857 	&	0.00006 	&	868	&	0.00251 	&	Kepler	\\
55382.89912 	&	0.00005 	&	871	&	0.00223 	&	Kepler	\\
55384.82020 	&	0.00007 	&	875	&	0.00219 	&	Kepler	\\
55386.26114 	&	0.00006 	&	878	&	0.00229 	&	Kepler	\\
55387.70173 	&	0.00019 	&	881	&	0.00204 	&	Kepler	\\
55389.14301 	&	0.00003 	&	884	&	0.00248 	&	Kepler	\\
55390.58360 	&	0.00009 	&	887	&	0.00222 	&	Kepler	\\
55392.02448 	&	0.00006 	&	890	&	0.00226 	&	Kepler	\\
55393.94579 	&	0.00007 	&	894	&	0.00245 	&	Kepler	\\
55395.38615 	&	0.00008 	&	897	&	0.00198 	&	Kepler	\\
55396.82740 	&	0.00007 	&	900	&	0.00239 	&	Kepler	\\
55398.26791 	&	0.00009 	&	903	&	0.00206 	&	Kepler	\\
55400.18932 	&	0.00011 	&	907	&	0.00235 	&	Kepler	\\
55402.11015 	&	0.00009 	&	911	&	0.00206 	&	Kepler	\\
55403.55105 	&	0.00006 	&	914	&	0.00212 	&	Kepler	\\
55404.99191 	&	0.00009 	&	917	&	0.00214 	&	Kepler	\\
55406.91304 	&	0.00010 	&	921	&	0.00215 	&	Kepler	\\
55408.35403 	&	0.00007 	&	924	&	0.00230 	&	Kepler	\\
55409.79467 	&	0.00009 	&	927	&	0.00210 	&	Kepler	\\
55411.23537 	&	0.00008 	&	930	&	0.00196 	&	Kepler	\\
55412.67645 	&	0.00009 	&	933	&	0.00221 	&	Kepler	\\
55414.11732 	&	0.00006 	&	936	&	0.00223 	&	Kepler	\\
55415.55813 	&	0.00009 	&	939	&	0.00221 	&	Kepler	\\
55416.99900 	&	0.00008 	&	942	&	0.00224 	&	Kepler	\\
55418.44001 	&	0.00007 	&	945	&	0.00240 	&	Kepler	\\
55420.36078 	&	0.00012 	&	949	&	0.00205 	&	Kepler	\\
55423.24249 	&	0.00008 	&	955	&	0.00209 	&	Kepler	\\
55425.16379 	&	0.00009 	&	959	&	0.00227 	&	Kepler	\\
55426.60487 	&	0.00012 	&	962	&	0.00251 	&	Kepler	\\
55428.04553 	&	0.00007 	&	965	&	0.00233 	&	Kepler	\\
55429.48607 	&	0.00007 	&	968	&	0.00202 	&	Kepler	\\
55431.88754 	&	0.00005 	&	973	&	0.00209 	&	Kepler	\\
55433.80902 	&	0.00005 	&	977	&	0.00246 	&	Kepler	\\
55435.24954 	&	0.00006 	&	980	&	0.00214 	&	Kepler	\\
55436.69048 	&	0.00006 	&	983	&	0.00224 	&	Kepler	\\
55438.13134 	&	0.00020 	&	986	&	0.00226 	&	Kepler	\\
55439.57238 	&	0.00018 	&	989	&	0.00246 	&	Kepler	\\
55441.01287 	&	0.00008 	&	992	&	0.00211 	&	Kepler	\\
55442.45376 	&	0.00007 	&	995	&	0.00216 	&	Kepler	\\
55444.37516 	&	0.00005 	&	999	&	0.00244 	&	Kepler	\\
55445.81574 	&	0.00009 	&	1002	&	0.00218 	&	Kepler	\\
55447.25674 	&	0.00006 	&	1005	&	0.00234 	&	Kepler	\\
55448.69762 	&	0.00011 	&	1008	&	0.00238 	&	Kepler	\\
55450.13843 	&	0.00008 	&	1011	&	0.00235 	&	Kepler	\\
55451.57907 	&	0.00010 	&	1014	&	0.00216 	&	Kepler	\\
55453.50011 	&	0.00022 	&	1018	&	0.00207 	&	Kepler	\\
55454.94091 	&	0.00009 	&	1021	&	0.00203 	&	Kepler	\\
55456.38191 	&	0.00011 	&	1024	&	0.00219 	&	Kepler	\\
55457.82280 	&	0.00008 	&	1027	&	0.00224 	&	Kepler	\\
55459.26354 	&	0.00009 	&	1030	&	0.00214 	&	Kepler	\\
55460.70418 	&	0.00009 	&	1033	&	0.00194 	&	Kepler	\\
55462.62579 	&	0.00010 	&	1037	&	0.00243 	&	Kepler	\\
55464.54659 	&	0.00007 	&	1041	&	0.00211 	&	Kepler	\\
55467.42858 	&	0.00023 	&	1047	&	0.00242 	&	Kepler	\\
55470.30992 	&	0.00007 	&	1053	&	0.00208 	&	Kepler	\\
55471.75091 	&	0.00007 	&	1056	&	0.00224 	&	Kepler	\\
55473.19145 	&	0.00007 	&	1059	&	0.00194 	&	Kepler	\\
55474.63249 	&	0.00008 	&	1062	&	0.00213 	&	Kepler	\\
55476.07329 	&	0.00008 	&	1065	&	0.00209 	&	Kepler	\\
55477.99450 	&	0.00007 	&	1069	&	0.00219 	&	Kepler	\\
55479.43532 	&	0.00006 	&	1072	&	0.00216 	&	Kepler	\\
55480.87567 	&	0.00005 	&	1075	&	0.00168 	&	Kepler	\\
55482.31662 	&	0.00006 	&	1078	&	0.00179 	&	Kepler	\\
55484.23840 	&	0.00005 	&	1082	&	0.00244 	&	Kepler	\\
55485.67919 	&	0.00005 	&	1085	&	0.00240 	&	Kepler	\\
55487.11990 	&	0.00006 	&	1088	&	0.00227 	&	Kepler	\\
55488.56066 	&	0.00006 	&	1091	&	0.00219 	&	Kepler	\\
55490.00134 	&	0.00008 	&	1094	&	0.00203 	&	Kepler	\\
55491.44214 	&	0.00007 	&	1097	&	0.00199 	&	Kepler	\\
55493.36347 	&	0.00007 	&	1101	&	0.00220 	&	Kepler	\\
55495.28429 	&	0.00008 	&	1105	&	0.00190 	&	Kepler	\\
55496.72479 	&	0.00023 	&	1108	&	0.00156 	&	Kepler	\\
55498.16661 	&	0.00008 	&	1111	&	0.00254 	&	Kepler	\\
55500.08731 	&	0.00007 	&	1115	&	0.00212 	&	Kepler	\\
55501.52831 	&	0.00007 	&	1118	&	0.00228 	&	Kepler	\\
55502.96911 	&	0.00011 	&	1121	&	0.00224 	&	Kepler	\\
55504.40989 	&	0.00012 	&	1124	&	0.00218 	&	Kepler	\\
55505.85087 	&	0.00008 	&	1127	&	0.00232 	&	Kepler	\\
55507.29178 	&	0.00008 	&	1130	&	0.00239 	&	Kepler	\\
55508.73261 	&	0.00010 	&	1133	&	0.00239 	&	Kepler	\\
55510.17343 	&	0.00006 	&	1136	&	0.00237 	&	Kepler	\\
55511.61400 	&	0.00009 	&	1139	&	0.00209 	&	Kepler	\\
55513.05513 	&	0.00009 	&	1142	&	0.00239 	&	Kepler	\\
55514.49586 	&	0.00008 	&	1145	&	0.00228 	&	Kepler	\\
55515.93656 	&	0.00007 	&	1148	&	0.00214 	&	Kepler	\\
55517.37753 	&	0.00005 	&	1151	&	0.00227 	&	Kepler	\\
55518.81809 	&	0.00008 	&	1154	&	0.00199 	&	Kepler	\\
55520.73931 	&	0.00006 	&	1158	&	0.00208 	&	Kepler	\\
55522.18031 	&	0.00007 	&	1161	&	0.00225 	&	Kepler	\\
55524.10125 	&	0.00005 	&	1165	&	0.00206 	&	Kepler	\\
55526.02231 	&	0.00013 	&	1169	&	0.00200 	&	Kepler	\\
55527.46304 	&	0.00005 	&	1172	&	0.00189 	&	Kepler	\\
55528.90441 	&	0.00011 	&	1175	&	0.00243 	&	Kepler	\\
55530.34482 	&	0.00007 	&	1178	&	0.00200 	&	Kepler	\\
55531.78588 	&	0.00006 	&	1181	&	0.00222 	&	Kepler	\\
55533.22652 	&	0.00007 	&	1184	&	0.00202 	&	Kepler	\\
55534.66754 	&	0.00007 	&	1187	&	0.00220 	&	Kepler	\\
55536.10816 	&	0.00007 	&	1190	&	0.00198 	&	Kepler	\\
55537.54901 	&	0.00005 	&	1193	&	0.00199 	&	Kepler	\\
55538.98989 	&	0.00007 	&	1196	&	0.00203 	&	Kepler	\\
55540.43085 	&	0.00006 	&	1199	&	0.00215 	&	Kepler	\\
55541.87158 	&	0.00007 	&	1202	&	0.00204 	&	Kepler	\\
55543.79290 	&	0.00005 	&	1206	&	0.00224 	&	Kepler	\\
55545.23362 	&	0.00006 	&	1209	&	0.00212 	&	Kepler	\\
55546.67472 	&	0.00011 	&	1212	&	0.00238 	&	Kepler	\\
55548.11518 	&	0.00010 	&	1215	&	0.00200 	&	Kepler	\\
55550.03694 	&	0.00013 	&	1219	&	0.00265 	&	Kepler	\\
55551.47722 	&	0.00009 	&	1222	&	0.00208 	&	Kepler	\\
55560.60259 	&	0.00009 	&	1241	&	0.00214 	&	Kepler	\\
55570.20810 	&	0.00007 	&	1261	&	0.00205 	&	Kepler	\\
55572.12910 	&	0.00061 	&	1265	&	0.00193 	&	Kepler	\\
55573.56990 	&	0.00009 	&	1268	&	0.00189 	&	Kepler	\\
55575.49109 	&	0.00005 	&	1272	&	0.00196 	&	Kepler	\\
55578.37302 	&	0.00005 	&	1278	&	0.00221 	&	Kepler	\\
55579.81389 	&	0.00008 	&	1281	&	0.00224 	&	Kepler	\\
55581.25392 	&	0.00006 	&	1284	&	0.00143 	&	Kepler	\\
55583.17545 	&	0.00006 	&	1288	&	0.00184 	&	Kepler	\\
55584.61612 	&	0.00008 	&	1291	&	0.00167 	&	Kepler	\\
55586.05723 	&	0.00007 	&	1294	&	0.00194 	&	Kepler	\\
55587.49809 	&	0.00010 	&	1297	&	0.00196 	&	Kepler	\\
55588.93885 	&	0.00009 	&	1300	&	0.00188 	&	Kepler	\\
55590.86087 	&	0.00019 	&	1304	&	0.00278 	&	Kepler	\\
55592.30086 	&	0.00008 	&	1307	&	0.00193 	&	Kepler	\\
55595.18315 	&	0.00009 	&	1313	&	0.00254 	&	Kepler	\\
55597.58388 	&	0.00009 	&	1318	&	0.00187 	&	Kepler	\\
55599.50523 	&	0.00008 	&	1322	&	0.00210 	&	Kepler	\\
55600.94597 	&	0.00008 	&	1325	&	0.00201 	&	Kepler	\\
55602.38703 	&	0.00009 	&	1328	&	0.00222 	&	Kepler	\\
55603.82772 	&	0.00010 	&	1331	&	0.00207 	&	Kepler	\\
55605.26853 	&	0.00008 	&	1334	&	0.00204 	&	Kepler	\\
55606.70934 	&	0.00012 	&	1337	&	0.00201 	&	Kepler	\\
55608.15077 	&	0.00014 	&	1340	&	0.00260 	&	Kepler	\\
55609.59097 	&	0.00011 	&	1343	&	0.00196 	&	Kepler	\\
55611.03182 	&	0.00006 	&	1346	&	0.00197 	&	Kepler	\\
55612.47287 	&	0.00009 	&	1349	&	0.00218 	&	Kepler	\\
55613.91367 	&	0.00008 	&	1352	&	0.00214 	&	Kepler	\\
55615.35431 	&	0.00017 	&	1355	&	0.00194 	&	Kepler	\\
55617.27571 	&	0.00008 	&	1359	&	0.00222 	&	Kepler	\\
55618.71624 	&	0.00007 	&	1362	&	0.00191 	&	Kepler	\\
55620.15767 	&	0.00006 	&	1365	&	0.00251 	&	Kepler	\\
55621.59874 	&	0.00013 	&	1368	&	0.00273 	&	Kepler	\\
55623.03889 	&	0.00017 	&	1371	&	0.00205 	&	Kepler	\\
55624.47982 	&	0.00014 	&	1374	&	0.00214 	&	Kepler	\\
55625.92067 	&	0.00006 	&	1377	&	0.00215 	&	Kepler	\\
55627.36130 	&	0.00007 	&	1380	&	0.00194 	&	Kepler	\\
55628.80218 	&	0.00006 	&	1383	&	0.00198 	&	Kepler	\\
55630.72354 	&	0.00008 	&	1387	&	0.00222 	&	Kepler	\\
55632.16403 	&	0.00006 	&	1390	&	0.00187 	&	Kepler	\\
55633.60528 	&	0.00006 	&	1393	&	0.00228 	&	Kepler	\\
55638.40787 	&	0.00013 	&	1403	&	0.00207 	&	Kepler	\\
55642.72990 	&	0.00008 	&	1412	&	0.00158 	&	Kepler	\\
55644.17087 	&	0.00009 	&	1415	&	0.00171 	&	Kepler	\\
55646.09230 	&	0.00009 	&	1419	&	0.00202 	&	Kepler	\\
55647.53282 	&	0.00011 	&	1422	&	0.00170 	&	Kepler	\\
55648.97385 	&	0.00007 	&	1425	&	0.00189 	&	Kepler	\\
55650.41459 	&	0.00009 	&	1428	&	0.00179 	&	Kepler	\\
55651.85570 	&	0.00009 	&	1431	&	0.00207 	&	Kepler	\\
55653.29612 	&	0.00049 	&	1434	&	0.00164 	&	Kepler	\\
55655.21765 	&	0.00012 	&	1438	&	0.00205 	&	Kepler	\\
55656.65842 	&	0.00006 	&	1441	&	0.00199 	&	Kepler	\\
55658.09924 	&	0.00023 	&	1444	&	0.00196 	&	Kepler	\\
55659.54044 	&	0.00011 	&	1447	&	0.00232 	&	Kepler	\\
55660.98092 	&	0.00014 	&	1450	&	0.00197 	&	Kepler	\\
55662.42185 	&	0.00009 	&	1453	&	0.00205 	&	Kepler	\\
55663.86254 	&	0.00010 	&	1456	&	0.00191 	&	Kepler	\\
55665.30339 	&	0.00006 	&	1459	&	0.00191 	&	Kepler	\\
55666.74441 	&	0.00010 	&	1462	&	0.00210 	&	Kepler	\\
55668.18512 	&	0.00007 	&	1465	&	0.00197 	&	Kepler	\\
55670.10642 	&	0.00008 	&	1469	&	0.00215 	&	Kepler	\\
55671.54730 	&	0.00008 	&	1472	&	0.00219 	&	Kepler	\\
55672.98818 	&	0.00008 	&	1475	&	0.00223 	&	Kepler	\\
55674.42890 	&	0.00008 	&	1478	&	0.00211 	&	Kepler	\\
55675.86977 	&	0.00007 	&	1481	&	0.00213 	&	Kepler	\\
55677.79079 	&	0.00010 	&	1485	&	0.00204 	&	Kepler	\\
55679.23178 	&	0.00009 	&	1488	&	0.00218 	&	Kepler	\\
55680.67243 	&	0.00006 	&	1491	&	0.00200 	&	Kepler	\\
55682.59366 	&	0.00007 	&	1495	&	0.00211 	&	Kepler	\\
55684.03450 	&	0.00006 	&	1498	&	0.00211 	&	Kepler	\\
55685.47521 	&	0.00007 	&	1501	&	0.00198 	&	Kepler	\\
55686.91632 	&	0.00008 	&	1504	&	0.00225 	&	Kepler	\\
55688.35677 	&	0.00005 	&	1507	&	0.00187 	&	Kepler	\\
55689.79767 	&	0.00007 	&	1510	&	0.00193 	&	Kepler	\\
55691.23849 	&	0.00006 	&	1513	&	0.00190 	&	Kepler	\\
55692.67947 	&	0.00005 	&	1516	&	0.00204 	&	Kepler	\\
55694.12008 	&	0.00007 	&	1519	&	0.00181 	&	Kepler	\\
55695.56123 	&	0.00010 	&	1522	&	0.00213 	&	Kepler	\\
55697.00177 	&	0.00008 	&	1525	&	0.00182 	&	Kepler	\\
55698.44272 	&	0.00005 	&	1528	&	0.00193 	&	Kepler	\\
55699.88350 	&	0.00007 	&	1531	&	0.00187 	&	Kepler	\\
55701.32414 	&	0.00008 	&	1534	&	0.00168 	&	Kepler	\\
55703.24553 	&	0.00009 	&	1538	&	0.00195 	&	Kepler	\\
55704.68616 	&	0.00014 	&	1541	&	0.00173 	&	Kepler	\\
55706.12721 	&	0.00010 	&	1544	&	0.00194 	&	Kepler	\\
55707.56778 	&	0.00010 	&	1547	&	0.00167 	&	Kepler	\\
55709.48871 	&	0.00008 	&	1551	&	0.00149 	&	Kepler	\\
55710.92988 	&	0.00007 	&	1554	&	0.00182 	&	Kepler	\\
55712.37048 	&	0.00008 	&	1557	&	0.00158 	&	Kepler	\\
55713.81166 	&	0.00006 	&	1560	&	0.00191 	&	Kepler	\\
55715.25218 	&	0.00012 	&	1563	&	0.00159 	&	Kepler	\\
55716.69354 	&	0.00006 	&	1566	&	0.00211 	&	Kepler	\\
55718.61451 	&	0.00008 	&	1570	&	0.00197 	&	Kepler	\\
55720.05514 	&	0.00019 	&	1573	&	0.00176 	&	Kepler	\\
55721.49597 	&	0.00009 	&	1576	&	0.00174 	&	Kepler	\\
55722.93714 	&	0.00010 	&	1579	&	0.00208 	&	Kepler	\\
55724.85796 	&	0.00010 	&	1583	&	0.00178 	&	Kepler	\\
55726.29879 	&	0.00008 	&	1586	&	0.00177 	&	Kepler	\\
55727.73970 	&	0.00010 	&	1589	&	0.00184 	&	Kepler	\\
55729.18074 	&	0.00007 	&	1592	&	0.00204 	&	Kepler	\\
55730.62138 	&	0.00009 	&	1595	&	0.00184 	&	Kepler	\\
55732.06232 	&	0.00007 	&	1598	&	0.00194 	&	Kepler	\\
55733.50311 	&	0.00007 	&	1601	&	0.00189 	&	Kepler	\\
55734.94405 	&	0.00006 	&	1604	&	0.00199 	&	Kepler	\\
55736.38507 	&	0.00009 	&	1607	&	0.00217 	&	Kepler	\\
55737.82566 	&	0.00007 	&	1610	&	0.00193 	&	Kepler	\\
55739.74687 	&	0.00008 	&	1614	&	0.00201 	&	Kepler	\\
55741.66790 	&	0.00009 	&	1618	&	0.00192 	&	Kepler	\\
55743.10883 	&	0.00008 	&	1621	&	0.00201 	&	Kepler	\\
55744.54969 	&	0.00014 	&	1624	&	0.00203 	&	Kepler	\\
55746.95124 	&	0.00005 	&	1629	&	0.00218 	&	Kepler	\\
55748.87212 	&	0.00006 	&	1633	&	0.00194 	&	Kepler	\\
55750.79345 	&	0.00008 	&	1637	&	0.00216 	&	Kepler	\\
55752.23402 	&	0.00008 	&	1640	&	0.00189 	&	Kepler	\\
55753.67508 	&	0.00009 	&	1643	&	0.00210 	&	Kepler	\\
55755.11581 	&	0.00007 	&	1646	&	0.00199 	&	Kepler	\\
55757.03703 	&	0.00005 	&	1650	&	0.00209 	&	Kepler	\\
55758.47789 	&	0.00005 	&	1653	&	0.00211 	&	Kepler	\\
55759.91858 	&	0.00005 	&	1656	&	0.00197 	&	Kepler	\\
55761.83966 	&	0.00008 	&	1660	&	0.00193 	&	Kepler	\\
55763.28052 	&	0.00006 	&	1663	&	0.00194 	&	Kepler	\\
55764.72185 	&	0.00012 	&	1666	&	0.00243 	&	Kepler	\\
55766.64237 	&	0.00008 	&	1670	&	0.00183 	&	Kepler	\\
55768.08330 	&	0.00007 	&	1673	&	0.00193 	&	Kepler	\\
55770.48452 	&	0.00008 	&	1678	&	0.00175 	&	Kepler	\\
55772.40573 	&	0.00007 	&	1682	&	0.00184 	&	Kepler	\\
55773.84679 	&	0.00006 	&	1685	&	0.00205 	&	Kepler	\\
55775.28752 	&	0.00011 	&	1688	&	0.00194 	&	Kepler	\\
55776.72815 	&	0.00012 	&	1691	&	0.00174 	&	Kepler	\\
55778.64974 	&	0.00016 	&	1695	&	0.00221 	&	Kepler	\\
55780.57083 	&	0.00003 	&	1699	&	0.00218 	&	Kepler	\\
55782.01143 	&	0.00009 	&	1702	&	0.00194 	&	Kepler	\\
55783.45255 	&	0.00010 	&	1705	&	0.00222 	&	Kepler	\\
55784.89327 	&	0.00015 	&	1708	&	0.00210 	&	Kepler	\\
55786.33408 	&	0.00007 	&	1711	&	0.00207 	&	Kepler	\\
55787.77442 	&	0.00009 	&	1714	&	0.00157 	&	Kepler	\\
55789.21585 	&	0.00009 	&	1717	&	0.00216 	&	Kepler	\\
55790.65644 	&	0.00011 	&	1720	&	0.00191 	&	Kepler	\\
55792.09708 	&	0.00011 	&	1723	&	0.00171 	&	Kepler	\\
55794.01870 	&	0.00006 	&	1727	&	0.00221 	&	Kepler	\\
55795.45940 	&	0.00006 	&	1730	&	0.00207 	&	Kepler	\\
55796.90022 	&	0.00006 	&	1733	&	0.00205 	&	Kepler	\\
55798.34112 	&	0.00010 	&	1736	&	0.00211 	&	Kepler	\\
55799.78184 	&	0.00005 	&	1739	&	0.00200 	&	Kepler	\\
55801.22300 	&	0.00011 	&	1742	&	0.00232 	&	Kepler	\\
55803.14368 	&	0.00006 	&	1746	&	0.00188 	&	Kepler	\\
55805.06497 	&	0.00006 	&	1750	&	0.00205 	&	Kepler	\\
55806.50584 	&	0.00007 	&	1753	&	0.00208 	&	Kepler	\\
55807.94652 	&	0.00008 	&	1756	&	0.00192 	&	Kepler	\\
55809.38746 	&	0.00005 	&	1759	&	0.00201 	&	Kepler	\\
55811.30849 	&	0.00005 	&	1763	&	0.00192 	&	Kepler	\\
55812.74935 	&	0.00006 	&	1766	&	0.00195 	&	Kepler	\\
55814.19002 	&	0.00007 	&	1769	&	0.00177 	&	Kepler	\\
55815.63086 	&	0.00005 	&	1772	&	0.00178 	&	Kepler	\\
55817.55231 	&	0.00007 	&	1776	&	0.00211 	&	Kepler	\\
55818.99271 	&	0.00009 	&	1779	&	0.00166 	&	Kepler	\\
55820.43385 	&	0.00007 	&	1782	&	0.00196 	&	Kepler	\\
55821.87443 	&	0.00007 	&	1785	&	0.00171 	&	Kepler	\\
55823.31546 	&	0.00005 	&	1788	&	0.00189 	&	Kepler	\\
55824.75618 	&	0.00011 	&	1791	&	0.00178 	&	Kepler	\\
55826.19699 	&	0.00009 	&	1794	&	0.00175 	&	Kepler	\\
55828.11896 	&	0.00009 	&	1798	&	0.00260 	&	Kepler	\\
55829.55896 	&	0.00008 	&	1801	&	0.00176 	&	Kepler	\\
55831.48022 	&	0.00009 	&	1805	&	0.00190 	&	Kepler	\\
55833.40141 	&	0.00008 	&	1809	&	0.00197 	&	Kepler	\\
55835.32250 	&	0.00009 	&	1813	&	0.00194 	&	Kepler	\\
55837.24384 	&	0.00007 	&	1817	&	0.00216 	&	Kepler	\\
55841.08611 	&	0.00010 	&	1825	&	0.00219 	&	Kepler	\\
55843.96776 	&	0.00010 	&	1831	&	0.00216 	&	Kepler	\\
55845.88930 	&	0.00010 	&	1835	&	0.00259 	&	Kepler	\\
55847.32948 	&	0.00008 	&	1838	&	0.00193 	&	Kepler	\\
55848.77062 	&	0.00007 	&	1841	&	0.00223 	&	Kepler	\\
55850.21136 	&	0.00006 	&	1844	&	0.00213 	&	Kepler	\\
55851.65211 	&	0.00006 	&	1847	&	0.00204 	&	Kepler	\\
55853.57360 	&	0.00008 	&	1851	&	0.00241 	&	Kepler	\\
55855.01416 	&	0.00010 	&	1854	&	0.00213 	&	Kepler	\\
55856.45514 	&	0.00006 	&	1857	&	0.00226 	&	Kepler	\\
55857.89583 	&	0.00006 	&	1860	&	0.00212 	&	Kepler	\\
55859.81689 	&	0.00007 	&	1864	&	0.00206 	&	Kepler	\\
55861.25792 	&	0.00008 	&	1867	&	0.00225 	&	Kepler	\\
55862.69860 	&	0.00007 	&	1870	&	0.00209 	&	Kepler	\\
55864.61966 	&	0.00007 	&	1874	&	0.00203 	&	Kepler	\\
55866.06108 	&	0.00007 	&	1877	&	0.00260 	&	Kepler	\\
55867.98167 	&	0.00007 	&	1881	&	0.00208 	&	Kepler	\\
55869.42254 	&	0.00007 	&	1884	&	0.00211 	&	Kepler	\\
55871.34349 	&	0.00008 	&	1888	&	0.00194 	&	Kepler	\\
55872.78446 	&	0.00008 	&	1891	&	0.00207 	&	Kepler	\\
55874.22507 	&	0.00009 	&	1894	&	0.00183 	&	Kepler	\\
55875.66609 	&	0.00005 	&	1897	&	0.00202 	&	Kepler	\\
55877.10686 	&	0.00012 	&	1900	&	0.00195 	&	Kepler	\\
55878.54766 	&	0.00008 	&	1903	&	0.00191 	&	Kepler	\\
55879.98859 	&	0.00013 	&	1906	&	0.00200 	&	Kepler	\\
55881.42943 	&	0.00008 	&	1909	&	0.00200 	&	Kepler	\\
55882.87033 	&	0.00007 	&	1912	&	0.00206 	&	Kepler	\\
55884.31111 	&	0.00006 	&	1915	&	0.00200 	&	Kepler	\\
55885.75213 	&	0.00012 	&	1918	&	0.00218 	&	Kepler	\\
55887.19279 	&	0.00008 	&	1921	&	0.00200 	&	Kepler	\\
55888.63361 	&	0.00008 	&	1924	&	0.00198 	&	Kepler	\\
55890.07432 	&	0.00008 	&	1927	&	0.00185 	&	Kepler	\\
55891.99562 	&	0.00007 	&	1931	&	0.00203 	&	Kepler	\\
55893.43660 	&	0.00009 	&	1934	&	0.00217 	&	Kepler	\\
55894.87734 	&	0.00008 	&	1937	&	0.00208 	&	Kepler	\\
55896.79854 	&	0.00006 	&	1941	&	0.00216 	&	Kepler	\\
55898.71956 	&	0.00007 	&	1945	&	0.00205 	&	Kepler	\\
55900.16053 	&	0.00006 	&	1948	&	0.00219 	&	Kepler	\\
55901.60130 	&	0.00005 	&	1951	&	0.00211 	&	Kepler	\\
55904.00286 	&	0.00008 	&	1956	&	0.00228 	&	Kepler	\\
55906.88441 	&	0.00004 	&	1962	&	0.00214 	&	Kepler	\\
55908.32513 	&	0.00005 	&	1965	&	0.00203 	&	Kepler	\\
55909.76614 	&	0.00004 	&	1968	&	0.00220 	&	Kepler	\\
55911.20688 	&	0.00006 	&	1971	&	0.00210 	&	Kepler	\\
55912.64769 	&	0.00008 	&	1974	&	0.00207 	&	Kepler	\\
55914.56904 	&	0.00010 	&	1978	&	0.00229 	&	Kepler	\\
55916.00962 	&	0.00006 	&	1981	&	0.00203 	&	Kepler	\\
55917.45059 	&	0.00006 	&	1984	&	0.00217 	&	Kepler	\\
55918.89121 	&	0.00008 	&	1987	&	0.00195 	&	Kepler	\\
55920.33224 	&	0.00005 	&	1990	&	0.00214 	&	Kepler	\\
55921.77300 	&	0.00008 	&	1993	&	0.00206 	&	Kepler	\\
55923.21389 	&	0.00007 	&	1996	&	0.00211 	&	Kepler	\\
55924.65462 	&	0.00010 	&	1999	&	0.00200 	&	Kepler	\\
55928.01692 	&	0.00010 	&	2006	&	0.00234 	&	Kepler	\\
55931.85901 	&	0.00065 	&	2014	&	0.00220 	&	Kepler	\\
55933.78016 	&	0.00008 	&	2018	&	0.00223 	&	Kepler	\\
55935.22061 	&	0.00010 	&	2021	&	0.00183 	&	Kepler	\\
55937.14227 	&	0.00012 	&	2025	&	0.00237 	&	Kepler	\\
55938.58253 	&	0.00010 	&	2028	&	0.00179 	&	Kepler	\\
55940.50395 	&	0.00006 	&	2032	&	0.00210 	&	Kepler	\\
55941.94481 	&	0.00006 	&	2035	&	0.00211 	&	Kepler	\\
55943.38529 	&	0.00008 	&	2038	&	0.00175 	&	Kepler	\\
55945.30647 	&	0.00009 	&	2042	&	0.00181 	&	Kepler	\\
55946.74760 	&	0.00009 	&	2045	&	0.00210 	&	Kepler	\\
55951.07007 	&	0.00006 	&	2054	&	0.00206 	&	Kepler	\\
55953.95188 	&	0.00007 	&	2060	&	0.00219 	&	Kepler	\\
55955.87268 	&	0.00012 	&	2064	&	0.00187 	&	Kepler	\\
55957.79397 	&	0.00006 	&	2068	&	0.00203 	&	Kepler	\\
55959.71519 	&	0.00007 	&	2072	&	0.00214 	&	Kepler	\\
55961.63565 	&	0.00010 	&	2076	&	0.00148 	&	Kepler	\\
55963.07768 	&	0.00011 	&	2079	&	0.00266 	&	Kepler	\\
55964.51775 	&	0.00006 	&	2082	&	0.00190 	&	Kepler	\\
55965.95909 	&	0.00011 	&	2085	&	0.00240 	&	Kepler	\\
55969.32063 	&	0.00020 	&	2092	&	0.00198 	&	Kepler	\\
55971.24147 	&	0.00011 	&	2096	&	0.00170 	&	Kepler	\\
55972.68294 	&	0.00093 	&	2099	&	0.00233 	&	Kepler	\\
55974.12368 	&	0.00011 	&	2102	&	0.00223 	&	Kepler	\\
55975.56439 	&	0.00009 	&	2105	&	0.00210 	&	Kepler	\\
55977.48595 	&	0.00019 	&	2109	&	0.00254 	&	Kepler	\\
55978.92640 	&	0.00013 	&	2112	&	0.00215 	&	Kepler	\\
55980.36785 	&	0.00014 	&	2115	&	0.00276 	&	Kepler	\\
55981.80823 	&	0.00013 	&	2118	&	0.00230 	&	Kepler	\\
55983.24908 	&	0.00011 	&	2121	&	0.00231 	&	Kepler	\\
55984.68975 	&	0.00013 	&	2124	&	0.00214 	&	Kepler	\\
55986.61079 	&	0.00008 	&	2128	&	0.00206 	&	Kepler	\\
55988.53169 	&	0.00010 	&	2132	&	0.00185 	&	Kepler	\\
55990.45321 	&	0.00008 	&	2136	&	0.00225 	&	Kepler	\\
55991.89380 	&	0.00011 	&	2139	&	0.00199 	&	Kepler	\\
55995.73614 	&	0.00009 	&	2147	&	0.00209 	&	Kepler	\\
55999.57803 	&	0.00008 	&	2155	&	0.00175 	&	Kepler	\\
56001.01897 	&	0.00009 	&	2158	&	0.00185 	&	Kepler	\\
56002.46005 	&	0.00008 	&	2161	&	0.00208 	&	Kepler	\\
56003.90034 	&	0.00008 	&	2164	&	0.00153 	&	Kepler	\\
56005.82199 	&	0.00008 	&	2168	&	0.00207 	&	Kepler	\\
56007.26279 	&	0.00007 	&	2171	&	0.00203 	&	Kepler	\\
56009.18415 	&	0.00006 	&	2175	&	0.00227 	&	Kepler	\\
56012.06564 	&	0.00012 	&	2181	&	0.00208 	&	Kepler	\\
56014.94757 	&	0.00006 	&	2187	&	0.00233 	&	Kepler	\\
56017.34904 	&	0.00004 	&	2192	&	0.00240 	&	Kepler	\\
56020.23049 	&	0.00009 	&	2198	&	0.00217 	&	Kepler	\\
56023.11249 	&	0.00009 	&	2204	&	0.00249 	&	Kepler	\\
56024.55298 	&	0.00010 	&	2207	&	0.00214 	&	Kepler	\\
56025.99393 	&	0.00006 	&	2210	&	0.00225 	&	Kepler	\\
56027.43467 	&	0.00011 	&	2213	&	0.00215 	&	Kepler	\\
56028.87581 	&	0.00009 	&	2216	&	0.00245 	&	Kepler	\\
56030.31644 	&	0.00008 	&	2219	&	0.00225 	&	Kepler	\\
56031.75743 	&	0.00007 	&	2222	&	0.00239 	&	Kepler	\\
56033.19815 	&	0.00010 	&	2225	&	0.00228 	&	Kepler	\\
56034.63886 	&	0.00008 	&	2228	&	0.00214 	&	Kepler	\\
56036.56040 	&	0.00009 	&	2232	&	0.00256 	&	Kepler	\\
56038.00106 	&	0.00011 	&	2235	&	0.00238 	&	Kepler	\\
56039.44203 	&	0.00012 	&	2238	&	0.00251 	&	Kepler	\\
56040.88268 	&	0.00011 	&	2241	&	0.00232 	&	Kepler	\\
56042.32356 	&	0.00007 	&	2244	&	0.00236 	&	Kepler	\\
56043.76454 	&	0.00010 	&	2247	&	0.00251 	&	Kepler	\\
56048.56713 	&	0.00006 	&	2257	&	0.00230 	&	Kepler	\\
56050.48844 	&	0.00014 	&	2261	&	0.00248 	&	Kepler	\\
56051.92914 	&	0.00008 	&	2264	&	0.00235 	&	Kepler	\\
56053.37000 	&	0.00007 	&	2267	&	0.00236 	&	Kepler	\\
56055.29114 	&	0.00008 	&	2271	&	0.00239 	&	Kepler	\\
56056.73188 	&	0.00007 	&	2274	&	0.00228 	&	Kepler	\\
56058.17279 	&	0.00008 	&	2277	&	0.00236 	&	Kepler	\\
56059.61354 	&	0.00006 	&	2280	&	0.00227 	&	Kepler	\\
56061.05426 	&	0.00008 	&	2283	&	0.00214 	&	Kepler	\\
56062.49541 	&	0.00007 	&	2286	&	0.00246 	&	Kepler	\\
56063.93612 	&	0.00009 	&	2289	&	0.00233 	&	Kepler	\\
56065.37672 	&	0.00010 	&	2292	&	0.00209 	&	Kepler	\\
56066.81772 	&	0.00006 	&	2295	&	0.00224 	&	Kepler	\\
56068.73906 	&	0.00006 	&	2299	&	0.00247 	&	Kepler	\\
56070.17954 	&	0.00007 	&	2302	&	0.00211 	&	Kepler	\\
56071.62062 	&	0.00009 	&	2305	&	0.00235 	&	Kepler	\\
56073.06140 	&	0.00008 	&	2308	&	0.00229 	&	Kepler	\\
56074.50232 	&	0.00005 	&	2311	&	0.00237 	&	Kepler	\\
56075.94298 	&	0.00004 	&	2314	&	0.00219 	&	Kepler	\\
56077.86454 	&	0.00019 	&	2318	&	0.00263 	&	Kepler	\\
56079.78545 	&	0.00006 	&	2322	&	0.00242 	&	Kepler	\\
56081.22610 	&	0.00008 	&	2325	&	0.00223 	&	Kepler	\\
56082.66700 	&	0.00006 	&	2328	&	0.00229 	&	Kepler	\\
56084.10813 	&	0.00007 	&	2331	&	0.00258 	&	Kepler	\\
56085.54882 	&	0.00006 	&	2334	&	0.00243 	&	Kepler	\\
56086.98982 	&	0.00011 	&	2337	&	0.00259 	&	Kepler	\\
56088.43070 	&	0.00009 	&	2340	&	0.00263 	&	Kepler	\\
56090.35152 	&	0.00008 	&	2344	&	0.00233 	&	Kepler	\\
56091.79264 	&	0.00010 	&	2347	&	0.00261 	&	Kepler	\\
56093.23333 	&	0.00009 	&	2350	&	0.00247 	&	Kepler	\\
56094.67430 	&	0.00009 	&	2353	&	0.00259 	&	Kepler	\\
56096.11500 	&	0.00010 	&	2356	&	0.00245 	&	Kepler	\\
56097.55597 	&	0.00008 	&	2359	&	0.00259 	&	Kepler	\\
56098.99676 	&	0.00011 	&	2362	&	0.00254 	&	Kepler	\\
56100.43764 	&	0.00007 	&	2365	&	0.00258 	&	Kepler	\\
56102.35887 	&	0.00007 	&	2369	&	0.00269 	&	Kepler	\\
56103.79953 	&	0.00010 	&	2372	&	0.00250 	&	Kepler	\\
56105.72089 	&	0.00008 	&	2376	&	0.00275 	&	Kepler	\\
56108.12200 	&	0.00007 	&	2381	&	0.00246 	&	Kepler	\\
56109.56275 	&	0.00008 	&	2384	&	0.00237 	&	Kepler	\\
56111.48378 	&	0.00008 	&	2388	&	0.00228 	&	Kepler	\\
56113.40496 	&	0.00009 	&	2392	&	0.00234 	&	Kepler	\\
56114.84563 	&	0.00006 	&	2395	&	0.00217 	&	Kepler	\\
56116.28657 	&	0.00009 	&	2398	&	0.00227 	&	Kepler	\\
56117.72752 	&	0.00009 	&	2401	&	0.00238 	&	Kepler	\\
56119.64848 	&	0.00007 	&	2405	&	0.00223 	&	Kepler	\\
56121.08943 	&	0.00009 	&	2408	&	0.00233 	&	Kepler	\\
56130.69510 	&	0.00007 	&	2428	&	0.00240 	&	Kepler	\\
56132.13571 	&	0.00005 	&	2431	&	0.00217 	&	Kepler	\\
56134.05692 	&	0.00005 	&	2435	&	0.00226 	&	Kepler	\\
56135.49791 	&	0.00004 	&	2438	&	0.00241 	&	Kepler	\\
56136.93853 	&	0.00004 	&	2441	&	0.00219 	&	Kepler	\\
56138.85963 	&	0.00006 	&	2445	&	0.00218 	&	Kepler	\\
56141.26148 	&	0.00005 	&	2450	&	0.00262 	&	Kepler	\\
56142.70237 	&	0.00006 	&	2453	&	0.00268 	&	Kepler	\\
56144.14303 	&	0.00005 	&	2456	&	0.00250 	&	Kepler	\\
56145.58378 	&	0.00008 	&	2459	&	0.00241 	&	Kepler	\\
56147.02489 	&	0.00004 	&	2462	&	0.00267 	&	Kepler	\\
56148.46535 	&	0.00007 	&	2465	&	0.00230 	&	Kepler	\\
56149.90633 	&	0.00006 	&	2468	&	0.00243 	&	Kepler	\\
56151.82758 	&	0.00005 	&	2472	&	0.00256 	&	Kepler	\\
56153.26846 	&	0.00007 	&	2475	&	0.00261 	&	Kepler	\\
56154.70922 	&	0.00005 	&	2478	&	0.00253 	&	Kepler	\\
56156.15008 	&	0.00011 	&	2481	&	0.00255 	&	Kepler	\\
56157.59095 	&	0.00006 	&	2484	&	0.00258 	&	Kepler	\\
56159.03169 	&	0.00008 	&	2487	&	0.00248 	&	Kepler	\\
56160.47267 	&	0.00008 	&	2490	&	0.00262 	&	Kepler	\\
56161.91350 	&	0.00007 	&	2493	&	0.00261 	&	Kepler	\\
56163.35447 	&	0.00008 	&	2496	&	0.00274 	&	Kepler	\\
56164.79512 	&	0.00011 	&	2499	&	0.00255 	&	Kepler	\\
56166.23587 	&	0.00007 	&	2502	&	0.00246 	&	Kepler	\\
56167.67682 	&	0.00006 	&	2505	&	0.00257 	&	Kepler	\\
56169.59815 	&	0.00006 	&	2509	&	0.00278 	&	Kepler	\\
56171.51893 	&	0.00007 	&	2513	&	0.00244 	&	Kepler	\\
56173.44017 	&	0.00007 	&	2517	&	0.00256 	&	Kepler	\\
56174.88083 	&	0.00008 	&	2520	&	0.00238 	&	Kepler	\\
56176.32167 	&	0.00007 	&	2523	&	0.00239 	&	Kepler	\\
56177.76244 	&	0.00007 	&	2526	&	0.00231 	&	Kepler	\\
56179.20338 	&	0.00008 	&	2529	&	0.00241 	&	Kepler	\\
56180.64431 	&	0.00009 	&	2532	&	0.00250 	&	Kepler	\\
56182.08503 	&	0.00007 	&	2535	&	0.00239 	&	Kepler	\\
56183.52581 	&	0.00005 	&	2538	&	0.00233 	&	Kepler	\\
56184.96676 	&	0.00007 	&	2541	&	0.00243 	&	Kepler	\\
56186.40731 	&	0.00010 	&	2544	&	0.00214 	&	Kepler	\\
56187.84849 	&	0.00007 	&	2547	&	0.00248 	&	Kepler	\\
56189.76957 	&	0.00005 	&	2551	&	0.00245 	&	Kepler	\\
56191.21032 	&	0.00007 	&	2554	&	0.00236 	&	Kepler	\\
56192.65134 	&	0.00006 	&	2557	&	0.00253 	&	Kepler	\\
56194.09195 	&	0.00007 	&	2560	&	0.00230 	&	Kepler	\\
56195.53298 	&	0.00006 	&	2563	&	0.00249 	&	Kepler	\\
56196.97357 	&	0.00006 	&	2566	&	0.00225 	&	Kepler	\\
56198.41452 	&	0.00005 	&	2569	&	0.00235 	&	Kepler	\\
56199.85523 	&	0.00008 	&	2572	&	0.00223 	&	Kepler	\\
56201.29635 	&	0.00007 	&	2575	&	0.00251 	&	Kepler	\\
56202.73703 	&	0.00010 	&	2578	&	0.00235 	&	Kepler	\\
56205.61877 	&	0.00074 	&	2584	&	0.00241 	&	Kepler	\\
56208.02035 	&	0.00007 	&	2589	&	0.00259 	&	Kepler	\\
56209.46112 	&	0.00009 	&	2592	&	0.00251 	&	Kepler	\\
56210.90204 	&	0.00006 	&	2595	&	0.00260 	&	Kepler	\\
56212.34280 	&	0.00010 	&	2598	&	0.00252 	&	Kepler	\\
56213.78378 	&	0.00008 	&	2601	&	0.00266 	&	Kepler	\\
56215.22450 	&	0.00011 	&	2604	&	0.00254 	&	Kepler	\\
56216.66533 	&	0.00008 	&	2607	&	0.00253 	&	Kepler	\\
56218.10617 	&	0.00004 	&	2610	&	0.00253 	&	Kepler	\\
56219.54698 	&	0.00007 	&	2613	&	0.00250 	&	Kepler	\\
56220.98785 	&	0.00008 	&	2616	&	0.00253 	&	Kepler	\\
56222.42862 	&	0.00007 	&	2619	&	0.00246 	&	Kepler	\\
56223.86957 	&	0.00008 	&	2622	&	0.00257 	&	Kepler	\\
56225.31029 	&	0.00007 	&	2625	&	0.00245 	&	Kepler	\\
56226.75126 	&	0.00008 	&	2628	&	0.00259 	&	Kepler	\\
56228.19189 	&	0.00006 	&	2631	&	0.00237 	&	Kepler	\\
56230.11287 	&	0.00006 	&	2635	&	0.00223 	&	Kepler	\\
56231.55397 	&	0.00006 	&	2638	&	0.00250 	&	Kepler	\\
56232.99463 	&	0.00007 	&	2641	&	0.00232 	&	Kepler	\\
56234.43577 	&	0.00004 	&	2644	&	0.00262 	&	Kepler	\\
56235.87639 	&	0.00008 	&	2647	&	0.00240 	&	Kepler	\\
56237.79763 	&	0.00007 	&	2651	&	0.00251 	&	Kepler	\\
56239.71858 	&	0.00006 	&	2655	&	0.00235 	&	Kepler	\\
56241.15957 	&	0.00006 	&	2658	&	0.00250 	&	Kepler	\\
56242.60019 	&	0.00008 	&	2661	&	0.00227 	&	Kepler	\\
56244.04131 	&	0.00005 	&	2664	&	0.00255 	&	Kepler	\\
56248.36359 	&	0.00007 	&	2673	&	0.00232 	&	Kepler	\\
56252.68617 	&	0.00007 	&	2682	&	0.00238 	&	Kepler	\\
56254.12714 	&	0.00007 	&	2685	&	0.00251 	&	Kepler	\\
56255.56781 	&	0.00007 	&	2688	&	0.00234 	&	Kepler	\\
56257.00900 	&	0.00007 	&	2691	&	0.00269 	&	Kepler	\\
56258.44950 	&	0.00007 	&	2694	&	0.00235 	&	Kepler	\\
56259.89068 	&	0.00010 	&	2697	&	0.00269 	&	Kepler	\\
56261.81172 	&	0.00008 	&	2701	&	0.00261 	&	Kepler	\\
56263.25264 	&	0.00007 	&	2704	&	0.00269 	&	Kepler	\\
56264.69348 	&	0.00009 	&	2707	&	0.00269 	&	Kepler	\\
56266.13424 	&	0.00007 	&	2710	&	0.00261 	&	Kepler	\\
56267.57518 	&	0.00007 	&	2713	&	0.00271 	&	Kepler	\\
56269.49595 	&	0.00007 	&	2717	&	0.00237 	&	Kepler	\\
56271.41748 	&	0.00007 	&	2721	&	0.00277 	&	Kepler	\\
56272.85813 	&	0.00007 	&	2724	&	0.00258 	&	Kepler	\\
56274.29903 	&	0.00007 	&	2727	&	0.00264 	&	Kepler	\\
56275.73984 	&	0.00009 	&	2730	&	0.00261 	&	Kepler	\\
56277.18078 	&	0.00007 	&	2733	&	0.00271 	&	Kepler	\\
56279.10182 	&	0.00005 	&	2737	&	0.00264 	&	Kepler	\\
56280.54261 	&	0.00006 	&	2740	&	0.00259 	&	Kepler	\\
56281.98357 	&	0.00005 	&	2743	&	0.00270 	&	Kepler	\\
56283.42426 	&	0.00006 	&	2746	&	0.00255 	&	Kepler	\\
56284.86522 	&	0.00004 	&	2749	&	0.00267 	&	Kepler	\\
56286.30588 	&	0.00005 	&	2752	&	0.00250 	&	Kepler	\\
56287.74692 	&	0.00006 	&	2755	&	0.00270 	&	Kepler	\\
56289.18747 	&	0.00006 	&	2758	&	0.00240 	&	Kepler	\\
56290.62845 	&	0.00006 	&	2761	&	0.00255 	&	Kepler	\\
56292.06922 	&	0.00006 	&	2764	&	0.00248 	&	Kepler	\\
56293.51013 	&	0.00006 	&	2767	&	0.00255 	&	Kepler	\\
56294.95082 	&	0.00007 	&	2770	&	0.00239 	&	Kepler	\\
56296.39179 	&	0.00006 	&	2773	&	0.00252 	&	Kepler	\\
56297.83234 	&	0.00008 	&	2776	&	0.00224 	&	Kepler	\\
56299.27332 	&	0.00007 	&	2779	&	0.00238 	&	Kepler	\\
56300.71399 	&	0.00010 	&	2782	&	0.00221 	&	Kepler	\\
56302.15497 	&	0.00008 	&	2785	&	0.00235 	&	Kepler	\\
56304.07630 	&	0.00013 	&	2789	&	0.00256 	&	Kepler	\\
56305.99733 	&	0.00007 	&	2793	&	0.00247 	&	Kepler	\\
56307.91847 	&	0.00009 	&	2797	&	0.00249 	&	Kepler	\\
56309.35945 	&	0.00011 	&	2800	&	0.00263 	&	Kepler	\\
56316.56382 	&	0.00007 	&	2815	&	0.00280 	&	Kepler	\\
56323.76822 	&	0.00008 	&	2830	&	0.00300 	&	Kepler	\\
56325.20869 	&	0.00005 	&	2833	&	0.00263 	&	Kepler	\\
56326.64965 	&	0.00008 	&	2836	&	0.00275 	&	Kepler	\\
56328.09028 	&	0.00005 	&	2839	&	0.00255 	&	Kepler	\\
56329.53140 	&	0.00006 	&	2842	&	0.00282 	&	Kepler	\\
56330.97198 	&	0.00007 	&	2845	&	0.00256 	&	Kepler	\\
56332.41272 	&	0.00004 	&	2848	&	0.00247 	&	Kepler	\\
56334.33428 	&	0.00005 	&	2852	&	0.00290 	&	Kepler	\\
56335.77489 	&	0.00007 	&	2855	&	0.00267 	&	Kepler	\\
56337.21591 	&	0.00005 	&	2858	&	0.00286 	&	Kepler	\\
56338.65649 	&	0.00005 	&	2861	&	0.00260 	&	Kepler	\\
56340.09750 	&	0.00005 	&	2864	&	0.00277 	&	Kepler	\\
56341.53821 	&	0.00006 	&	2867	&	0.00264 	&	Kepler	\\
56342.97915 	&	0.00006 	&	2870	&	0.00274 	&	Kepler	\\
56344.41993 	&	0.00008 	&	2873	&	0.00268 	&	Kepler	\\
56345.86079 	&	0.00006 	&	2876	&	0.00269 	&	Kepler	\\
56347.30138 	&	0.00008 	&	2879	&	0.00244 	&	Kepler	\\
56348.74238 	&	0.00007 	&	2882	&	0.00261 	&	Kepler	\\
56350.66355 	&	0.00006 	&	2886	&	0.00266 	&	Kepler	\\
56352.10416 	&	0.00008 	&	2889	&	0.00243 	&	Kepler	\\
56353.54517 	&	0.00007 	&	2892	&	0.00259 	&	Kepler	\\
56354.98594 	&	0.00010 	&	2895	&	0.00253 	&	Kepler	\\
56356.42685 	&	0.00007 	&	2898	&	0.00260 	&	Kepler	\\
56358.34774 	&	0.00008 	&	2902	&	0.00237 	&	Kepler	\\
56360.74927 	&	0.00012 	&	2907	&	0.00250 	&	Kepler	\\
56362.19018 	&	0.00006 	&	2910	&	0.00257 	&	Kepler	\\
56363.63101 	&	0.00010 	&	2913	&	0.00256 	&	Kepler	\\
56365.07184 	&	0.00006 	&	2916	&	0.00255 	&	Kepler	\\
56366.51296 	&	0.00008 	&	2919	&	0.00283 	&	Kepler	\\
56367.95344 	&	0.00007 	&	2922	&	0.00248 	&	Kepler	\\
56369.87451 	&	0.00009 	&	2926	&	0.00242 	&	Kepler	\\
56371.31563 	&	0.00008 	&	2929	&	0.00270 	&	Kepler	\\
56372.75642 	&	0.00006 	&	2932	&	0.00265 	&	Kepler	\\
56374.19754 	&	0.00014 	&	2935	&	0.00293 	&	Kepler	\\
56375.63817 	&	0.00007 	&	2938	&	0.00272 	&	Kepler	\\
56377.07911 	&	0.00007 	&	2941	&	0.00283 	&	Kepler	\\
56378.51974 	&	0.00006 	&	2944	&	0.00261 	&	Kepler	\\
56380.44101 	&	0.00006 	&	2948	&	0.00277 	&	Kepler	\\
56381.88194 	&	0.00006 	&	2951	&	0.00286 	&	Kepler	\\
56383.32268 	&	0.00005 	&	2954	&	0.00276 	&	Kepler	\\
56384.76347 	&	0.00005 	&	2957	&	0.00271 	&	Kepler	\\
56386.20430 	&	0.00005 	&	2960	&	0.00270 	&	Kepler	\\
56387.64532 	&	0.00005 	&	2963	&	0.00287 	&	Kepler	\\
56389.08600 	&	0.00005 	&	2966	&	0.00271 	&	Kepler	\\
56391.48714 	&	0.00033 	&	2971	&	0.00246 	&	Kepler	\\
56393.40863 	&	0.00005 	&	2975	&	0.00283 	&	Kepler	\\
56394.84937 	&	0.00008 	&	2978	&	0.00273 	&	Kepler	\\
56396.29037 	&	0.00004 	&	2981	&	0.00289 	&	Kepler	\\
56397.73104 	&	0.00007 	&	2984	&	0.00272 	&	Kepler	\\
56399.17208 	&	0.00004 	&	2987	&	0.00292 	&	Kepler	\\
56400.61268 	&	0.00007 	&	2990	&	0.00268 	&	Kepler	\\
56402.05366 	&	0.00006 	&	2993	&	0.00282 	&	Kepler	\\
56403.49432 	&	0.00006 	&	2996	&	0.00264 	&	Kepler	\\
56404.93534 	&	0.00007 	&	2999	&	0.00282 	&	Kepler	\\
56406.37603 	&	0.00007 	&	3002	&	0.00267 	&	Kepler	\\
56407.81698 	&	0.00005 	&	3005	&	0.00278 	&	Kepler	\\
56409.25765 	&	0.00008 	&	3008	&	0.00262 	&	Kepler	\\
56410.69866 	&	0.00006 	&	3011	&	0.00278 	&	Kepler	\\
56412.13950 	&	0.00008 	&	3014	&	0.00278 	&	Kepler	\\
56413.58027 	&	0.00006 	&	3017	&	0.00271 	&	Kepler	\\
56417.90256 	&	0.00013 	&	3026	&	0.00248 	&	Kepler	\\
56421.74488 	&	0.00010 	&	3034	&	0.00257 	&	Kepler	\\
56423.18581 	&	0.00007 	&	3037	&	0.00265 	&	Kepler	\\
56788.21816 	&	0.00182 	&	3797	&	0.02228 	&	ASAS\-SN	\\
56836.70650 	&	0.00114 	&	3898	&	0.00235 	&	ASAS\-SN	\\
56836.71712 	&	0.00114 	&	3898	&	0.01297 	&	ASAS\-SN	\\
56924.60113 	&	0.00156 	&	4081	&	0.00575 	&	ASAS\-SN	\\
56924.61174 	&	0.00156 	&	4081	&	0.01637 	&	ASAS\-SN	\\
57119.11032 	&	0.00126 	&	4486	&	0.00159 	&	ASAS\-SN	\\
57119.12093 	&	0.00126 	&	4486	&	0.01220 	&	ASAS\-SN	\\
57193.55501 	&	0.00087 	&	4641	&	0.00290 	&	ASAS\-SN	\\
57193.56563 	&	0.00087 	&	4641	&	0.01351 	&	ASAS\-SN	\\
57258.87302 	&	0.00120 	&	4777	&	0.00283 	&	ASAS\-SN	\\
57258.88363 	&	0.00120 	&	4777	&	0.01345 	&	ASAS\-SN	\\
57497.09360 	&	0.00168 	&	5273	&	0.00458 	&	ASAS\-SN	\\
57497.10421 	&	0.00168 	&	5273	&	0.01520 	&	ASAS\-SN	\\
57560.97016 	&	0.00115 	&	5406	&	0.00392 	&	ASAS\-SN	\\
57560.98077 	&	0.00115 	&	5406	&	0.01453 	&	ASAS\-SN	\\
57633.01375 	&	0.00170 	&	5556	&	0.00552 	&	ASAS\-SN	\\
57633.02436 	&	0.00170 	&	5556	&	0.01613 	&	ASAS\-SN	\\
57860.18524 	&	0.00176 	&	6029	&	0.00462 	&	ASAS\-SN	\\
57860.19585 	&	0.00176 	&	6029	&	0.01523 	&	ASAS\-SN	\\
57918.29750 	&	0.00101 	&	6150	&	0.00301 	&	ASAS\-SN	\\
57918.30811 	&	0.00101 	&	6150	&	0.01363 	&	ASAS\-SN	\\
57981.21315 	&	0.00152 	&	6281	&	0.00200 	&	ASAS\-SN	\\
57981.22376 	&	0.00152 	&	6281	&	0.01261 	&	ASAS\-SN	\\
58293.41551 	&	0.00136 	&	6931	&	0.02242 	&	ASAS\-SN	\\
58684.83233 	&	0.00014 	&	7746	&	0.01112 	&	TESS	\\
58687.23309 	&	0.00030 	&	7751	&	0.01049 	&	TESS	\\
58689.63502 	&	0.00019 	&	7756	&	0.01101 	&	TESS	\\
58692.03671 	&	0.00015 	&	7761	&	0.01130 	&	TESS	\\
58694.43752 	&	0.00017 	&	7766	&	0.01071 	&	TESS	\\
58697.31929 	&	0.00024 	&	7772	&	0.01081 	&	TESS	\\
58700.20134 	&	0.00014 	&	7778	&	0.01118 	&	TESS	\\
58702.60349 	&	0.00047 	&	7783	&	0.01193 	&	TESS	\\
58705.48388 	&	0.00019 	&	7789	&	0.01064 	&	TESS	\\
58707.88561 	&	0.00023 	&	7794	&	0.01097 	&	TESS	\\
58712.68863 	&	0.00019 	&	7804	&	0.01119 	&	TESS	\\
58715.08994 	&	0.00023 	&	7809	&	0.01110 	&	TESS	\\
58717.49198 	&	0.00020 	&	7814	&	0.01174 	&	TESS	\\
58719.89384 	&	0.00019 	&	7819	&	0.01220 	&	TESS	\\
58722.29447 	&	0.00024 	&	7824	&	0.01143 	&	TESS	\\
58725.65662 	&	0.00028 	&	7831	&	0.01163 	&	TESS	\\
58728.53833 	&	0.00039 	&	7837	&	0.01166 	&	TESS	\\
58730.93937 	&	0.00019 	&	7842	&	0.01129 	&	TESS	\\
58733.34078 	&	0.00024 	&	7847	&	0.01130 	&	TESS	\\
58735.74265 	&	0.00022 	&	7852	&	0.01177 	&	TESS	\\
59391.80545 	&	0.00018 	&	9218	&	0.01223 	&	TESS	\\
59394.20696 	&	0.00017 	&	9223	&	0.01234 	&	TESS	\\
59396.60817 	&	0.00016 	&	9228	&	0.01215 	&	TESS	\\
59399.48987 	&	0.00014 	&	9234	&	0.01218 	&	TESS	\\
59401.89157 	&	0.00014 	&	9239	&	0.01247 	&	TESS	\\
59404.77331 	&	0.00015 	&	9245	&	0.01254 	&	TESS	\\
59407.65504 	&	0.00018 	&	9251	&	0.01258 	&	TESS	\\
59410.05644 	&	0.00016 	&	9256	&	0.01259 	&	TESS	\\
59412.45785 	&	0.00031 	&	9261	&	0.01259 	&	TESS	\\
59414.85913 	&	0.00015 	&	9266	&	0.01248 	&	TESS	\\
59417.26068 	&	0.00014 	&	9271	&	0.01262 	&	TESS	\\
59421.10296 	&	0.00018 	&	9279	&	0.01267 	&	TESS	\\
59423.50430 	&	0.00019 	&	9284	&	0.01261 	&	TESS	\\
59425.90565 	&	0.00020 	&	9289	&	0.01256 	&	TESS	\\
59428.78759 	&	0.00019 	&	9295	&	0.01282 	&	TESS	\\
59431.18871 	&	0.00020 	&	9300	&	0.01254 	&	TESS	\\
59434.07069 	&	0.00020 	&	9306	&	0.01284 	&	TESS	\\
59436.95209 	&	0.00018 	&	9312	&	0.01256 	&	TESS	\\
59439.35360 	&	0.00019 	&	9317	&	0.01267 	&	TESS	\\
59441.75478 	&	0.00017 	&	9322	&	0.01245 	&	TESS	\\
59444.63615 	&	0.00018 	&	9328	&	0.01215 	&	TESS	\\
59745.29243 	&	0.00042 	&	9954	&	0.01321 	&	TESS	\\
59747.69398 	&	0.00035 	&	9959	&	0.01336 	&	TESS	\\
59750.09535 	&	0.00020 	&	9964	&	0.01333 	&	TESS	\\
59752.49673 	&	0.00016 	&	9969	&	0.01331 	&	TESS	\\
59755.37853 	&	0.00028 	&	9975	&	0.01343 	&	TESS	\\
59758.26007 	&	0.00035 	&	9981	&	0.01329 	&	TESS	\\
59760.66148 	&	0.00027 	&	9986	&	0.01330 	&	TESS	\\
59763.54321 	&	0.00017 	&	9992	&	0.01335 	&	TESS	\\
59765.94437 	&	0.00016 	&	9997	&	0.01311 	&	TESS	\\
\hline\hline
\end{tabular}
\end{center}
\end{table}

